On the Interaction of Adaptive Population Control with Cumulative Step-Size Adaptation

Three state-of-the-art adaptive population control strategies (PCS) are theoretically and empirically investigated for a multi-recombinative, cumulative step-size adaptation Evolution Strategy $(\mu/\mu_I, \lambda)$-CSA-ES. First, scaling properties for the generation number and mutation strength rescaling are derived on the sphere in the limit of large population sizes. Then, the adaptation properties of three standard CSA-variants are studied as a function of the population size and dimensionality, and compared to the predicted scaling results. Thereafter, three PCS are implemented along the CSA-ES and studied on a test bed of sphere, random, and Rastrigin functions. The CSA-adaptation properties significantly influence the performance of the PCS, which is shown in more detail. Given the test bed, well-performing parameter sets (in terms of scaling, efficiency, and success rate) for both the CSA- and PCS-subroutines are identified.

==> alg_csa.tex <==
\begin{algorithm}[t]
	\caption{$(\mu/\mu_I, \lambda)$-CSA-ES with generic population control strategy (PCS)}
	\label{alg:alg1}
	\begin{algorithmic}[1]
		\State $g \gets 0$ 
		\State $\operatorname{initialize\_csa\_es}\qty(\vb{y}^{(0)}, \vb{s}^{(0)}, \sigma^{(0)}, c_\sigma, d_\sigma, D)$ %\vb{y}^{(0)}, \sigma^{(0)}, \vb{s}^{(0)}, c_\sigma, d_\sigma, D
		\State $\operatorname{initialize\_pcs}(\textit{method-specific})$ (Sec.~\cref{sec:pcs})
		\Repeat
		\For{$l = 1, ..., \lambda$} 
		\State $\tilde{\vb{z}}_l \gets [\mathcal{N}(0,1), ..., \mathcal{N}(0,1)]$
		\State $\tilde{\vb{y}}_l \gets \vb{y}^{(g)} + \sigma^{(g)}\tilde{\vb{z}}_l$ 
		\State $\tilde{f}_l \gets f(\vb{\tilde{y}}_l)$
		\EndFor
		\State	$(\tilde{f}_{1;\lambda}, ..., \tilde{f}_{m;\lambda}, ..., \tilde{f}_{\mu;\lambda} ) \gets \operatorname{sort}(\tilde{f}_1, ..., \tilde{f}_\lambda )$
		\State $\vb{y}^{(g+1)} \gets \frac{1}{\mu}\SUMM \tilde{\vb{y}}_{m;\lambda}$ 
		\State $\rec{\vb{z}}^{(g+1)} \gets \frac{1}{\mu}\SUMM \vb{z}_{m;\lambda}$
		\State $\vb{s}^{(g+1)} \gets (1-c_\sigma)\vb{s}^{(g)} + \sqrt{\mu c_\sigma(2-c_\sigma)}\rec{\vb{z}}^{(g+1)}$
		\State $\sigma^{(g+1)} \gets \text{update via \cref{eq:new_han_v1} or \cref{eq:neq_han_v2}}$
		\State $\mu^{(g+1)} \gets \mathrm{pcs(\mu^{(g)},\textit{method-specific})} \text{ (Sec.~\cref{sec:pcs})}$
		\State $\sigma^{(g+1)} \gets \mathrm{sigma\_rescale(\mu^{(g)},\mu^{(g+1)})}$
		\State $g \gets g+1$
		\Until termination criterion
	\end{algorithmic}
\end{algorithm}%

==> cmds_old.tex <==
% Format
\newcommand{\mycomment}[1]{}
\newcommand{\myind}[0]{}
\newcommand{\myindplus}[0]{\qquad}
\newcommand{\ParR}[1]{\left(#1\right)}
\newcommand{\ParE}[1]{\left[#1\right]}
\newcommand{\ym}[1]{\colorbox{yellow!30}{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\rsp}[1]{\,{#1}\,}

% Abbreviations ES
\newcommand{\ESmuLam}[0]{(\mu/\mu_I, \lambda)\text{-ES}}
\newcommand{\SUMM}[0]{\sum_{m=1}^{\mu}}
\newcommand{\SUMNEQ}[0]{\sum_{j \neq i}}
\newcommand{\CMULAM}[0]{c_{\mu/\mu,\lambda}}
\newcommand{\CTHETA}[0]{c_{\vartheta}}
\newcommand{\CTHETAlong}[0]{\ONETWOPI \frac{1}{\vartheta} \EXP{ -\frac{1}{2} \ParR{\Phi^{-1}(\vartheta)}^2 }}

% Abbreviations ES: y, phi1, phi2
\newcommand{\yig}[0]{y_i^{(g)}}
\newcommand{\yigp}[0]{y_i^{(g+1)}}
\newcommand{\ybg}[0]{\vb{y}^{(g)}}
\newcommand{\ybgp}[0]{\vb{y}^{(g+1)}}
\newcommand{\phiI}[0]{\varphi_i}
\newcommand{\phiII}[0]{\varphi_i^{\mathrm{II}}}
\newcommand{\phiR}[0]{\varphi^{\mathrm{II}}_R}
\newcommand{\phiRnorm}[0]{\varphi^{\mathrm{II,*}}_R}
\newcommand{\phiSphNorm}[0]{\varphi^*_\mathrm{sph}}

% Abbreviations Misc
\newcommand{\Ninf}[0]{N \rightarrow \infty}
\newcommand{\ONETWOPI}[1][]{\frac{1}{\sqrt{2\pi}#1}}
\newcommand{\OVMU}[0]{\frac{1}{\mu}}
\newcommand{\OVMUsq}[0]{\frac{1}{\mu^2}}
\newcommand{\fpi}[0]{f'_i}

% Operators General
\newcommand{\e}[0]{\mathrm{e}}
\newcommand{\EXP}[1]{\operatorname{exp}\left[ #1 \right]}
\newcommand{\He}[2]{\operatorname{He}_{#1}\ParR{#2}}
\newcommand{\FH}[0]{\operatorname{F}}
\newcommand{\FHYP}[1][-k]{\operatorname{F}\left( #1, \lambda-\mu, \lambda, 1/\that \right)}
\newcommand{\GAM}[1]{\operatorname{\Gamma}(#1)}
\newcommand{\BET}[1]{\operatorname{B}(#1)}
\newcommand{\TAYLORvI}[3]{\sum_{k=0}^{\infty} \frac{1}{k!} \left. \pdv[k]{#1}{#2} \right\rvert_{#2=#3}(#2-#3)^{k}}
\newcommand{\SGN}[1]{\operatorname{sgn}\ParR{#1}}
\newcommand{\BigO}[1]{O\ParR{#1}}
\newcommand{\SmO}[1]{o\ParR{#1}}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

% Operators Statistics
\newcommand{\EV}[1]{\operatorname{E}\left[#1\right]}
\newcommand{\VAR}[1]{\operatorname{Var}\left[#1\right]}
\newcommand{\EVC}[2]{\operatorname{E}\left[#1|#2\right]}
\newcommand{\EVCspace}[2]{\operatorname{E}\left[\,#1\,\big|\,#2\,\right]}
\newcommand{\VARC}[2]{\operatorname{Var}\left[#1|#2\right]}
\newcommand{\OV}[1]{\overline{#1}}
\newcommand{\NORMCDF}[2]{\Phi \left(\frac{#1}{#2} \right)}
\newcommand{\NORMPDF}[2]{\frac{1}{\sqrt{2\pi}#2} \EXP{-\frac{1}{2}\left(\frac{#1}{#2}\right)^2}}
\newcommand{\STDNORMPDF}[2]{\frac{1}{#2}\phi\ParR{\frac{#1}{#2}}}
\newcommand{\NORMPDFshort}[2]{\frac{1}{\sqrt{2\pi}#2} \e^{-\frac{1}{2}\left(\frac{#1}{#2}\right)^2}}

\newcommand{\mean}[0]{\mathrm{mean}}
\newcommand{\median}[0]{\mathrm{median}}

% Abbrev. Statistics
\newcommand{\expfac}[2]{\e^{-{\frac{1}{2}\frac{#1^2}{#2^2}}}}
\newcommand{\expfacParR}[2]{\e^{-\frac{1}{2}\left(\frac{#1}{#2}\right)^2}}
\newcommand{\expfacSingle}[1]{\e^{-{\frac{1}{2}{#1^2}}}}

% Random variables
\newcommand{\RANDVAR}[3]{ #1 \sim \mathcal{N}\ParR{#2,#3^2} }
\newcommand{\RANDStdNorm}[1]{ #1 \sim \mathcal{N}(0,1) }
\newcommand{\RANDU}[3]{ #1 \sim \mathcal{U}([#2,#3]) }
\newcommand{\RANDN}[2]{\mathcal{N}\ParR{#1,#2^2} }

% Abbrev. Rastrigin
\newcommand{\ci}[0]{A\myc{y_i}}
\newcommand{\si}[0]{A\mys{y_i}}

% ----- Expected value of Quality Gain -----
\newcommand{\EQi}[0]{E_{Q_i}}
\newcommand{\Ei}[0]{E_{i}}
\newcommand{\Di}[0]{D_{i}}
\newcommand{\Qxy}[0]{Q_{\vb{y}}(\vb{x})}
\newcommand{\QxyTilde}[0]{\wt{Q}_{\vb{y}}(\vb{x})}
\newcommand{\EQyxi}[0]{E_{Q|x_i}}
\newcommand{\DQyxi}[0]{\Di}%{D_{Q|x_i}}
\newcommand{\QiNonLin}[0]{x_i^2 +  2y_i x_i +c_i(1-\myc{x_i}) + s_i\mys{x_i}}
\newcommand{\EQiLONG}[0]{ \sigma^2 + \ci \left(1-\evcSH\right) }

% D_Q^2 Formula
\newcommand{\evprefac}{\e^{-\frac{1}{2} (\alpha \sigma)^2}}
\newcommand{\evprefacNOHALF}{\e^{-(\alpha \sigma)^2}}
\newcommand{\evprefacII}{\e^{-\frac{1}{2} (\alpha s)^2}}

% -----
\newcommand{\QGainResTI}[0]{4 \sigma^2 y_i^2  + 2\sigma^4} 
\newcommand{\QGainResTII}[0]{\frac{A^2}{2}\ParR{1-\evprefacNOHALF}\ParR{1-\cos(2 \alpha y_i)\evprefacNOHALF}}
\newcommand{\QGainResTIII}[0]{2 A \alpha \sigma^2 \evprefac \Big( \alpha \sigma^2 \cos(\alpha y_i) + 2y_i\sin(\alpha y_i) \Big)}
%V1: \newcommand{\QGainResTI}[0]{2\sigma^4 + 4 y_i^2 \sigma^2 + \frac{A^2}{2}\ParE{1-\evprefacNOHALF}}
%V1: \newcommand{\QGainResTII}[0]{\frac{A^2}{2} \evprefacNOHALF \cos(2 \alpha y_i) \ParE{\evprefacNOHALF-1}}
%V1: \newcommand{\QGainResTIII}[0]{2 A \alpha \sigma^2 \evprefac \Big[ \alpha \sigma^2 \cos(\alpha y_i) + 2y_i\sin(\alpha y_i) \Big]}
 
 % Custom trigonometric functions
\newcommand{\myc}[1]{\cos{\left( \alpha#1 \right)}}
\newcommand{\mycc}[1]{\cos^2{\left( \alpha#1 \right)}}
\newcommand{\mys}[1]{\sin{\left( \alpha#1 \right)}}
\newcommand{\myss}[1]{\sin^2{\left( \alpha#1 \right)}}
\newcommand{\myxs}[1]{#1\sin{\left( \alpha#1 \right)}}
\newcommand{\myxxc}[1]{#1^2\cos{\left( \alpha#1 \right)}}

% Long versions
\newcommand{\evc}{\operatorname{exp}\left[{-\frac{1}{2}(\alpha\sigma)^2}\right] }
\newcommand{\evcc}{\frac{1}{2}\left(1 + \operatorname{exp}\left[{-\frac{1}{2}(2\alpha\sigma)^2}\right]\right)}
\newcommand{\evss}{\frac{1}{2}\left(1 - \operatorname{exp}\left[{-\frac{1}{2}(2\alpha\sigma)^2}\right]\right)}
\newcommand{\evxxc}{(\sigma^2 - \alpha^2 \sigma^4) \evc}
\newcommand{\evxs}{\alpha \sigma^2 \evc}

% Short versions
\newcommand{\evcSH}{\e^{-\frac{(\alpha\sigma)^2}{2}}}
\newcommand{\evccSH}{\frac{1}{2} + \frac{1}{2}\e^{-\frac{(2\alpha\sigma)^2}{2}}}
\newcommand{\evssSH}{\frac{1}{2} - \frac{1}{2}\e^{-\frac{(2\alpha\sigma)^2}{2}}}
%\newcommand{\evcSH}{\e^{-(\alpha\sigma)^2/2}}
\newcommand{\evxsSH}{\alpha \sigma^2 \evcSH}
\newcommand{\evxxcSH}{(\sigma^2 - \alpha^2 \sigma^4) \evcSH}
\newcommand{\varsinSH}{\frac{1 - \e^{-2(\alpha\sigma)^2}}{2}}
\newcommand{\varcosSH}{\frac{1 + \e^{-2(\alpha\sigma)^2} - 2\e^{-(\alpha\sigma)^2}}{2}}

% Specific commands for progress rates
\newcommand{\PHIinvVar}[0]{\Phi^{-1}(\vartheta)}
\newcommand{\OneOverBetaFactor}[0]{\frac{(\lambda-1)!}{(\lambda-\mu-1)!(\mu-1)!}}
\newcommand{\prefacMdep}[0]{\frac{\lambda!}{(m-1)!(\lambda-m)!}}

\newcommand{\xmLam}[0]{x_{m;\lambda}}
\newcommand{\xkLam}[0]{x_{k;\lambda}}
\newcommand{\xlLam}[0]{x_{l;\lambda}}
\newcommand{\zlLam}[0]{z_{l;\lambda}}
\newcommand{\zkLam}[0]{z_{k;\lambda}}
\newcommand{\zmLam}[0]{z_{m;\lambda}}
\newcommand{\ARSIG}[2]{\zeta_{#1}^{(#2)}}
\newcommand{\pJointDensNu}[0]{p_{n_1, ..., n_\nu;\lambda}(z_1, ..., z_\nu)}
\newcommand{\pJointDensNuTransf}[0]{p^*_{n_1, ..., n_\nu;\lambda}(z^*_1, ..., z^*_\nu)}
\newcommand{\piPermSum}[0]{\pi_P(z_{n_1;\lambda}, ..., z_{n_\nu;\lambda})}
\newcommand{\piPermSumTransf}[0]{\pi_P(z^*_{n_1;\lambda}, ..., z^*_{n_\nu;\lambda})}
\newcommand{\facPermTransf}[0]{(-1)^{\norm{P}_1}}

\newcommand{\pmx}[0]{p_{m;\lambda}(x_i|\vb{y})}
\newcommand{\pqxy}[0]{p_Q(q | x_i, \vb{y})}
\newcommand{\pqx}[0]{p_Q(q | x_i)}
\newcommand{\Pqy}[0]{P_Q(q | \vb{y})}
\newcommand{\PPinv}[0]{P_Q(\Pqinv | x_i)}
\newcommand{\Pq}[0]{P_Q(q)}
\newcommand{\Pqinv}[0]{P_Q^{-1}(1-t)}

\newcommand{\tOneMinT}[0]{t^{\lambda-\mu-1}(1-t)^{\mu-1}}
\newcommand{\xOneMinX}[3]{\left[ #1 \right]^{#2}\left[ 1-#1 \right]^{#3}}
\newcommand{\that}[0]{\hat{t}}
%\newcommand{\Dk}[0]{{\widetilde{\sigma}\mkern 0mu}}
\newcommand{\factorEqDqI}[0]{\EXP{ -\frac{1}{2} \left(\frac{ \EQi+D_Q \Phi^{-1}(\vartheta) }{\Dk}\right)^2 }}
\newcommand{\Dk}[0]{D_{+}}
\newcommand{\Df}[0]{D_{f}}
\newcommand{\cZero}[0]{\frac{ \EQi+D_Q \Phi^{-1}(\vartheta)}{\Di}}
\newcommand{\mAfterQuadComp}[0]{\frac{ [\EQi+D_Q \Phi^{-1}(\vartheta)]k_i\sigma^2 }{\Dk^2}}
\newcommand{\sAfterQuadComp}[0]{\frac{D_i\sigma}{\Dk}}
\newcommand{\CAfterQuadComp}[0]{\factorEqDqI}
\newcommand{\sigeps}[0]{\sigma_\epsilon}

\newcommand{\kapv}[0]{\widetilde{\kappa}}%{\kappa^{(v)}}
\newcommand{\gamv}[0]{\widetilde{\gamma}}%{\gamma^{(v)}}

\newcommand{\sigN}[0]{(\sigma^*/N)}
\newcommand{\Nsig}[0]{(N/\sigma^*)}

\newcommand{\limVartheta}[2]{\lim_{\begin{subarray}{l} #1 \rightarrow \infty \\ \vartheta = \text{const.}\end{subarray}}{#2}}

%% Specific commands phi_i^II
\newcommand{\sigRN}[0]{\sigma^*\frac{R}{N}}
\newcommand{\sigNormSph}[0]{\hat{\sigma}^*_{\text{sph}}}

%% Specific commands dynamical systems & iteration
\newcommand{\y}[1]{y_{#1}}
\newcommand{\RR}[1]{r_{#1}}
\newcommand{\myphi}[0]{\varphi^{*}}

%% SAR
\newcommand{\vs}[0]{\varsigma}
\newcommand{\vt}[0]{\vartheta}

%% New misc commands
\newcommand{\signss}[0]{\sigma^*_{\mathrm{ss}}}
\newcommand{\signzero}[0]{\sigma^*_{\varphi_0}}
\newcommand{\sigpsizero}[0]{\sigma_{\psi_0}}
\newcommand{\signsec}[0]{\sigma^*_{\mathrm{sec}}}
\newcommand{\signcr}[0]{\sigma^*_{\mathrm{crit}}}
\newcommand{\phiNormSph}[0]{\varphi^*_{\mathrm{sph}}}
\newcommand{\rec}[1]{\langle#1\rangle}
\newcommand{\limvt}[0]{\lim_{\begin{subarray}{1}\mu,\lambda \rightarrow \infty \\ \vartheta = \mathrm{const.}\end{subarray}}}
\newcommand{\SALN}[0]{\sigma\text{SA}_L}
\newcommand{\SAEP}[0]{\sigma\text{SA}_N}

%% Population control
\newcommand{\Per}[0]{\mathcal{P}}
\newcommand{\Thr}[0]{\mathcal{T}}
\newcommand{\Mag}[0]{\mathcal{M}}
